Type System for Four Delimited Control Operators

The operational behavior of control operators has been studied comprehensively in the past few decades, but type systems of control operators have not. There are distinct type systems for shift, control, and shift0 without any relationship between them, and there has not been a type system that directly corresponds to control0. This paper remedies this situation by giving a uniform type system for all the four control operators. Following Danvy and Filinski's approach, we derive a monomorphic type system from the CPS interpreter that defines the operational semantics of the four control operators. By implementing the typed CPS interpreter in Agda, we show that the CPS translation preserves types and that the calculus with all the four control operators is terminating. Furthermore, we show the relationship between our type system and the previous type systems for shift, control, and shift0.

==> Makefile <==
.SUFFIXES: .tex .pdf .all

.DELETE_ON_ERROR:

all :
	@echo usage: make filename.all / make clean

.tex.all :
	pdflatex $<
	bibtex $*
	pdflatex $<
	pdflatex $<

.tex.pdf :
	pdflatex $<
	if grep "No file $*.bbl." $*.log ||\
	   grep 'There were undefined references.' $*.log ||\
	   grep 'There were undefined citations.' $*.log ;\
	then\
	  bibtex $* ;\
	  pdflatex $< ;\
	fi
	while grep 'Rerun to get ' $*.log ; do\
	  pdflatex $< ;\
	done

clean :
	rm -f *.ps *.bak *.dvi *.aux *.log *.toc *.idx *.nav *.out *.snm *.vrb *.ptb *.ilg *.ind *.bbl *.blg *.pag *.vtc

-include .depend


==> review.tex <==
GPCE 2022 Paper #12 Reviews and Comments
===========================================================================
Paper #12 Type System for Four Delimited Control Operators


Review #12A
===========================================================================

Overall merit
-------------
4. Accept

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
This paper proposes a monomorphic calculus $\lambda_D$
(with a type system and a CPS interpreter) for four control operators:
`shift`, `shift0`, `control`, and `control0`.
The translation from $\lambda_D$ to the target language $\lambda_C$
preserves types and terminates (proved in Agda).
While `shift` is often used with `reset`, and `control` is paired with
`prompt`, in $\lambda_D$, `reset` and `prompt` are unified,
after which the dynamic semantics of the four control operators
`shift`, `shift0`, `control`, and `control0` only differ
in a very subtle way.
The claimed contributions of the paper are (1) giving the first typing rule
for `control0` (which supports answer type modification) and
(2) subsuming the existing three type systems for `shift`, `shift0`,
and `control`; therefore $\lambda_D$ could serve as a foundation
for further investigation.

Comments for author
-------------------
Pros:
- The paper is well written and the code is well documented.
- The systems and most of the proofs are formalized in Agda

Cons:
- The introduction and comparison of these four operators is
relatively short. E.g. L67 says they can be classified by
"static" and "dynamic" but this discussion is not elaborated later.
In general I feel the motivation of modeling these operators and
especially why answer type modification is important are not well explained.
- Part of the proofs is not mechanized (L1153 footnote is not even proved).

From a non-expert perspective, this paper seems interesting,
with technical depth and I would be inclined to accept it.
Nonetheless, there are some questions on whether the choice of
these four operators is adequate and whether the delta of the paper
is sufficient over previous work.
Perhaps other reviewers can say more about that.

Comments:

- L114 (Sec. 2): The examples and reduction rules helped me understanding the behaviors of the operators. I will appreciate if there are more examples comparing these operators and explaining the impacts of delimiters. I am also curious how to type-check such concrete examples in later technical sections (if the space allows).

- L224 (Fig. 1): $\alpha$ and $\beta$ are not introduced. Are they just like $\tau$?

- L335: $\varepsilon[[e]]$ in Fig. 3 denotes the CPS translation of $e$, right? The notation seems to be a bit misleading as $\varepsilon$ often corresponds to an evaluation context.

- L423 (Sec. 4): As $\lambda_D$ is similar to the calculus of Cong et al. [7] (i.e. CP in 5.2), it would be better to explain the changes in the typing rules a bit.

Review #12B
===========================================================================

Overall merit
-------------
4. Accept

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This paper presents a single type system for four known
delimited-control operators, shift, shift0, control, and control0 and
studies its properties and relationship to other type systems (for a
single operator).

The type system is obtained from a CPS translation, similarly to Danvy
and Filinski's work on a type system for shift: the conditions that
the interpretation of a term of a certain form (such as, abstraction,
application and so on) is well typed are considered the conditions for
the original term to be well typed.  The CPS translation is proved to
be type preserving; as a byproduct of the fact that the target
language is STLC, termination of the source language is obtained as an
easy consequence.

As for comparisons with existing type systems for control operators,
Danvi and Filinski's type system for shift/reset, Cong et al.'s type
system for control/prompt, and Materzok and Biercnacki's type system
for shift0/reset0 are discussed.  They are basically special cases of
the proposed type system (although differences in how entities like
meta-continuations are represented in the (CPS) semantics make the
development more complicated) and the proposed type system is shown to
be equivalent in terms of typability.

The main results (except for a few theorems, whose pencil-and-paper
proofs are given in Appendix) are formalized in Agda.

Comments for author
-------------------
Pros:

* Solid work on a unifying type system for the known four delimited-control operators.
* Relationship to existing type systems is clearly discussed.
* The main theorems are formalized in Agda.

Cons:

* (The presentation of) the technical development should have been
  less puzzling.

Delimited control operators have been studied in the context of
computational effects and their applications include program
transformation/code generation.  The subject of the present paper,
which is a type system for delimited control operators, might not be
typical of GPCE but I think it is still relevant.

Although the presented type system is rather compilicated, it seems it
is the price to pay to deal with the nature of these control operators
in one system.  I'm impressed by the author(s), who carried out the
entire development in Agda, raising the level of credibility of the
technical development.

The paper is overall well written.  The introduction to four
delimited-control operators is gentle and nice.  The typing rules look
scary but their derivations are well explained by using the CPS
semantics and still accessible.  Section 5 on the comparisons with
other type systems are dense (because three type systems are compared)
but informally described key ideas help understanding.  Although I
must say I haven't checked details, the results are convincing and
plausible.

I found the CPS interpreter in Figure 3 puzzling, however, because the
target language is set to be STLC with the unit and pair types but the
definition of $k_{id}$ doesn't look like a well typed STLC-term.  I
thought $k_{id}$ might be a meta-level function (just like
$\mathcal{E}$) but found some of the uses of $\kappa$ contradicted my
guess -- for example, in the defining clause for variables, $\kappa$
is applied to $\rho(x)$, $t$, and $m$ but $t$ and $m$ are object-level
variables and I had no idea what happens if $\kappa$ is $k_{id}$.  So,
the CPS interpreter didn't make much sense to me (until reading the
paper a few times).

I think the real definition of $k_{id}$ (as an STLC term) depends on
some type information, namely, it is an STLC term of type $\gamma_1^*
\rightarrow \mu^* \rightarrow \sigma^* \rightarrow \gamma_2^*$ where
$\mathsf{id-cont-type}(\gamma_1, \mu, \sigma, \gamma_2)$ holds.  For
example, if $\mu = \bullet$ and $\sigma = \bullet$ and $\gamma_1 =
\gamma_2$, then $k_{id} = \lambda v. \lambda (). \lambda (). v$.  It
seems to me that, for the CPS interpreter in Figure 3 to be
well-defined, it has to be defined as a function from well typed terms
or, more precisely, a function from type devirations.  (I think this
is not the case for Danvy and Filinski's type system for shift/reset.)


### Minor comments

* The first item of the contribution list (on p. 1) is not really
  presented.

* p.3: "In general, the interpreter takes ... and evaluate[s] the term e"

* p.6, "The goal of this section is to show that if a term e is
  typable in DF, then e is also typable in 4D": The converse (which is
  shown eventually) is also important, I guess?

Review #12C
===========================================================================

Overall merit
-------------
5. Strong accept

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
The paper presents a new unified type system for a language with four related control operators (shift, control, shift0, control0).  The type system is systematically derived from a double-CPS interpreter (with both a continuation and a metacontinuation).  The whole system is formalised in Agda, as are various typeability connections between the authors' system and existing systems for typing delimited control.

Comments for author
-------------------
+ Valuable contribution that supports typing four related delimited control operators in a single system
+ Well-written and well-structured paper that repays careful reading
+ Systematic derivation of the type system from an interpreter
+ Clean PHOAS-based formalisation in Agda provided as supplementary material
+ Thorough comparison with previous (mostly simpler) work, drawing close connections
+ Exciting (and plausible) future work on extending to richer forms of delimited control (e.g. answer type polymorphism) and algebraic effects

- Complex typing judgment (but perhaps unavoidably so)

Suggestion: it'd be helpful to have the order of control operators on lines 131-134 match the order elsewhere (e.g. Figure 3)

Question: might there be a useful interpretation of your type system as a logic (i.e. via the Curry-Howard isomorphism)?

------------------------
## Author Response

Thank you all for your valuable feedback. We will respond to each review below.

-----
For the review 12A:

At L224 (Figure 1), $\alpha$ and $\beta$ are value and term types. They are basically the same as $\tau$, but they often represent answer types.
Also, at L335, $\mathcal{E}[\![e]\!]$ denotes CPS interpreter and is not an evaluation context.
We should add some descriptions of the notations to avoid confusion.

-----
For the review 12B:

Thanks to your comment, we noticed that the definition of $k_{id}$ in Figure 3 does not type check in $\lambda_{C}$ (STLC + unit + pair). While reviewing the definition, we also realized that we have properly implemented it in Agda just as you described.
Similarly, the definition of trail composition ($\_@\_$ and $\_::\_$) on the paper needs additional type information.

The type of $k_{id}$ and trail composition ($\_@\_$ and $\_::\_$) should be below:
  * $k_{id} : \forall \tau,\tau',\mu,\sigma.\,\textsf{id-cont-type}(\tau,\mu,\sigma,\tau')\to\tau^*\to\mu^*\to\sigma^*\to\tau'^*$
  * both $\_@\_$ and $\_::\_$ : $\forall \mu_1,\mu_2,\mu_3.\,\textsf{compatible}(\mu_1,\mu_2,\mu_3)\to\mu_1^*\to\mu_2^*\to\mu_3^*$

In accordance with above definitions, each line of $\mathcal{S},\mathcal{F},\mathcal{S_0},\mathcal{F_0}$ in $\mathcal{E}[\![\,]\!]$ should receive $\textsf{id-cont-type}$ and/or $\textsf{compatible}$.

We think the description should reflect exactly what was implemented. Since the definitions of $\textsf{id-cont-type}$ and $\textsf{compatible}$ are presented in subsequent sections, we will try to rewrite the paragraph so that the reader can understand.


-----
For the review 12C:

As for the interpretation of our type system from a logical point of view, we do not have one yet at this time. It would be interesting to further understand the system as future work.

